On string topology of classifying spaces

Let G be a compact Lie group. By work of Chataur and Menichi, the homology of the space of free loops in the classifying space of G is known to be the value on the circle in a homological conformal field theory. This means in particular that it admits operations parameterized by homology classes of classifying spaces of diffeomorphism groups of surfaces. Here we present a radical extension of this result, giving a new construction in which diffeomorphisms are replaced with homotopy equivalences, and surfaces with boundary are replaced with arbitrary spaces homotopy equivalent to finite graphs. The result is a novel kind of field theory which is related to both the diffeomorphism groups of surfaces and the automorphism groups of free groups with boundaries. Our work shows that the algebraic structures in string topology of classifying spaces can be brought into line with, and in fact far exceed, those available in string topology of manifolds. For simplicity, we restrict to the characteristic 2 case. The generalization to arbitrary characteristic will be addressed in a subsequent paper.

==> declarations.tex <==
\usepackage{amsfonts, amssymb, amsmath, eucal, amsthm, stmaryrd, verbatim}
\usepackage[all,cmtip]{xy}
\xyoption{ps}
\xyoption{dvips}
\usepackage{mathtools}

\newcounter{dummy}

\makeatletter

% Formatting
%\usepackage{mathptmx}
\DeclareSymbolFont{cmlargesymbols}{OMX}{cmex}{m}{n}
%\usepackage[vmargin=3.2cm, hmargin=3.4cm]{geometry}
%\usepackage[vmargin=3.2cm, hmargin=3.4cm]{geometry}
\usepackage[vmargin=3.2cm]{geometry}
%\parindent=12pt
%\parskip=6pt plus3pt minus3pt

\usepackage{color}
\usepackage{hyperref}  
\hypersetup{%
  bookmarksnumbered=true,%
%  bookmarks=true,%
  colorlinks=true,%
  linkcolor=blue,%
  citecolor=blue,%
  filecolor=blue,%
  menucolor=blue,%
%  pagecolor=blue,%
  urlcolor=blue,%
  pdfnewwindow=true,%
  pdfstartview=}
%\usepackage{txfonts}


%\usepackage[notref,notcite]{showkeys}
\usepackage{threeparttable}
%\usepackage{booktabs}


% marginal notes e.g. \mnote{blah blah}
\newcommand\mnote[1]{\marginpar{\tiny #1}}
\setlength{\marginparsep}{0.2cm}
\setlength{\marginparwidth}{2.5cm}
\setlength{\marginparpush}{0.5cm}

\newcommand{\acomment}[1]{\footnote{#1}}

%Environment Definitions:

\newtheorem{lemma}{Lemma}
\newtheorem{theorem}[lemma]{Theorem}
\newtheorem*{theorem*}{Theorem}
\newtheorem{proposition}[lemma]{Proposition}
\newtheorem{corollary}[lemma]{Corollary}
\newtheorem{conjecture}[lemma]{Conjecture}
\newtheorem*{maintheorem}{Theorem A}
\newtheorem*{cmtheorem}{Theorem B}

\theoremstyle{definition}
\newtheorem{definition}[lemma]{Definition}
\newtheorem{note}[lemma]{Note}
\newtheorem{example}[lemma]{Example}
\newtheorem{examples}[lemma]{Examples}
\newtheorem{remark}[lemma]{Remark}
\newtheorem*{remark*}{Remark}
\newtheorem{question}[lemma]{Question}
\newtheorem*{acknowledgments}{Acknowledgments}
\newtheorem{notation}[lemma]{Notation}
\newtheorem{construction}[lemma]{Construction}
\numberwithin{lemma}{section}

\newtheorem{step}{Step}

%Symbol Commands:

\newcommand{\g}{\mathfrak{g}}
\newcommand{\Diff}{\mathrm{Diff}}
\newcommand{\Homeo}{\mathrm{Homeo}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\pt}{\mathrm{pt}}
\newcommand{\free}{\mathrm{free}}
\newcommand{\OC}{{\mathcal{OC}}}
\newcommand{\Vect}{\mathrm{Vect}}
\newcommand{\Fun}{\mathrm{Fun}}
\newcommand{\ad}{\mathrm{ad}}
\newcommand{\Ad}{\mathrm{Ad}}
\newcommand{\Map}{\mathrm{Map}}
\newcommand{\Cyl}{\mathrm{Cyl}}
\newcommand{\vertical}{\mathrm{vert}}
\newcommand{\hAut}{\mathrm{hAut}}
\newcommand{\Aut}{\mathrm{Aut}}
\newcommand{\Hol}{\mathrm{Hol}}
\newcommand{\rmin}{\mathit{in}}
\newcommand{\rmout}{\mathit{out}}
\newcommand{\rmfree}{\mathit{free}}

\newcommand{\Godin}{\mathrm{Gdn}}
\newcommand{\CM}{\mathrm{CM}}

\newcommand{\bp}{\mathrm{bp}}
\newcommand{\hg}{\mathrm{hg}}
\newcommand{\ds}{\mathrm{ds}}
\newcommand{\mfld}{\mathrm{man}}

\DeclareMathOperator{\Ob}{Ob}
\DeclareMathOperator{\Mor}{Mor}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\cod}{cod}
\DeclareMathOperator{\Sing}{Sing}

\newcommand{\N}{\mathbf{N}}
\newcommand{\Z}{\mathbf{Z}}
\newcommand{\Q}{\mathbf{Q}}
\newcommand{\R}{\mathbf{R}}
\newcommand{\C}{\mathbf{C}}
\newcommand{\T}{\mathbb{T}}

\newcommand{\gpdI}{\calI} % The groupoid with two objects 
                          % 0 and 1 and a unique isomorphism
                          % between them.
\newcommand{\Pifw}{\Pi^\mathrm{fw}}


\newcommand{\parman}{{\bbM\mathbf{an}}}
\newcommand{\parmanvvb}{\parman^{\mathrm{vvb}}}
\newcommand{\parmanlc}{\parman^{\mathrm{lc}}}
\newcommand{\parmanvvbfincw}{\parman^{\mathrm{vvb,finCW}}}
\newcommand{\parmanlcfincw}{\parman^{\mathrm{lc,finCW}}}
\newcommand{\sq}{\bbS\mathbf{q}}

\newcommand{\parhg}{{\mathbb{H}\mathbf{G}}}
\newcommand{\parhglc}{\parhg^\mathrm{lc}}
\newcommand{\parhglcbp}{\parhg^\mathrm{lc,bp}}

\newcommand{\pargpd}{{\mathbb{G}\mathbf{pd}}}
\newcommand{\pargpdlc}{\pargpd^\mathrm{lc}}

\newcommand{\PP}{\mathbb{PP}}
\newcommand{\tw}{\mathit{tw}}

\newcommand{\grmod}{\mathbf{grMod}}
\newcommand{\modmod}{{\slash\!\!\slash}} % Like \sslash, but with better spacing.
\renewcommand{\sslash}{\modmod}

\newcommand{\fun}{\mathrm{fun}}




%%% Arrows

% Slashed arrows, based on Andrew Stacey's code at
%
% http://tex.stackexchange.com/questions/13938/how-do-i-create-the-negated-arrow-on-xrightarrow
%
% and Shulman's decls.tex.
\def\slashedarrowfill@#1#2#3#4#5{%
  $\m@th\thickmuskip0mu\medmuskip\thickmuskip\thinmuskip\thickmuskip
   \relax#5#1\mkern-7mu%
   \cleaders\hbox{$#5\mkern-2mu#2\mkern-2mu$}\hfill
   \mathclap{#3}\mathclap{#2}%
   \cleaders\hbox{$#5\mkern-2mu#2\mkern-2mu$}\hfill
   \mkern-7mu#4$%
}
\def\rightslashedarrowfill@{%
  \slashedarrowfill@\relbar\relbar\mapstochar\rightarrow}
\newcommand\xhto[2][]{%
  \ext@arrow 1579{\rightslashedarrowfill@}{#1}{#2}}

\newcommand{\hto}{\xhto{}}

% Replacement for xrightarrow, with shorter name and 
% the same spacing as the slashed arrow above.
\newcommand\xto[2][]{%
  \ext@arrow 1579{\rightarrowfill@}{#1}{#2}}

\newcommand\xot[2][]{%
  \ext@arrow 5197{\leftarrowfill@}{#1}{#2}}

% Long versions
\newcommand{\longhto}{\xhto{\quad}}
\newcommand{\longto}{\xto{\quad}}
\newcommand{\longot}{\xot{\quad}}

\newcommand{\longincl}{\xhookrightarrow{\quad}}
\newcommand{\longrevincl}{\xhookleftarrow{\quad}}

% I copied here a number of commands I have grown used to using. 
% Please feel free to edit as you wish. -A

\newcommand{\tensor}{\otimes}
\newcommand{\smashprod}{\wedge}

\newcommand{\id}{\mathrm{id}}
\newcommand{\Id}{\mathrm{Id}}

\newcommand{\isom}{\approx}
\newcommand{\homot}{\simeq}
\newcommand{\nhomot}{\not\simeq}
\newcommand{\homeom}{\approx}

\newcommand{\suspension}{\Sigma}
\newcommand{\loops}{\Omega}

\newcommand{\bdry}{\partial}

%\newcommand{\ho}{\mathrm{Ho}\,} % Notation for homotopy category
\DeclareMathOperator{\ho}{Ho} % Notation for homotopy category

\newcommand{\invlim}{\varprojlim}
\newcommand{\dirlim}{\varinjlim}

\newcommand{\incl}{\hookrightarrow}
\newcommand{\goesto}{\xrightarrow}
\newcommand{\cl}[1]{\overline{#1}} %closure

\DeclareMathOperator{\colim}{colim}
\newcommand{\im}{\mathrm{Im}\,}
\providecommand{\ker}{}
\renewcommand{\ker}{\mathrm{Ker}\,}
\DeclareMathOperator{\interior}{int}
\DeclareMathOperator{\diam}{diam}

\newcommand{\ev}{\mathrm{ev}}
\newcommand{\pr}{\mathrm{pr}}
\newcommand{\foldmap}{\nabla}

\newcommand{\VB}{\mathbf{VB}}     % vector bundles
\newcommand{\vVB}{\mathbf{vVB}}   % virtual bundles

\newcommand{\umk}{\shortleftarrow} % decoration for umkerh maps



% Notation for our double categories

\newcommand{\cob}{\mathbb{C}\mathbf{ob}}
\newcommand{\cobbp}{\cob^{\mathrm{bp}}}
\newcommand{\gpd}{\mathbb{G}}
\newcommand{\man}{\mathbb{M}}
\newcommand{\pmor}{\mathbb{P}\mathbf{Mor}}

% Notation for 2-categories

\newcommand{\Cat}{\mathcal{C}\mathit{at}} % 2-cat of categories
\newcommand{\Dbl}{\mathcal{D}\mathit{bl}} % 2-cat of double categories
\newcommand{\Fib}{\mathcal{F}\mathit{ib}} % 2-cat of fibrations

% Opposites
\newcommand{\co}{\mathrm{co}} % reverse 2-morphisms
\newcommand{\op}{\mathrm{op}}
\newcommand{\hop}{\mathrm{hop}}
\newcommand{\fop}{\mathrm{fop}}



%%% Blackboard bold letters

\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}

%%% Calligraphic letters

\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}

%%% Fraktur letters

\newcommand{\fA}{\mathfrak{A}}
\newcommand{\fB}{\mathfrak{B}}
\newcommand{\fC}{\mathfrak{C}}
\newcommand{\fD}{\mathfrak{D}}
\newcommand{\fE}{\mathfrak{E}}
\newcommand{\fF}{\mathfrak{F}}
\newcommand{\fG}{\mathfrak{G}}
\newcommand{\fH}{\mathfrak{H}}
\newcommand{\fI}{\mathfrak{I}}
\newcommand{\fJ}{\mathfrak{J}}
\newcommand{\fK}{\mathfrak{K}}
\newcommand{\fL}{\mathfrak{L}}
\newcommand{\fM}{\mathfrak{M}}
\newcommand{\fN}{\mathfrak{N}}
\newcommand{\fO}{\mathfrak{O}}
\newcommand{\fP}{\mathfrak{P}}
\newcommand{\fQ}{\mathfrak{Q}}
\newcommand{\fR}{\mathfrak{R}}
\newcommand{\fS}{\mathfrak{S}}
\newcommand{\fT}{\mathfrak{T}}
\newcommand{\fU}{\mathfrak{U}}
\newcommand{\fV}{\mathfrak{V}}
\newcommand{\fW}{\mathfrak{W}}
\newcommand{\fX}{\mathfrak{X}}
\newcommand{\fY}{\mathfrak{Y}}
\newcommand{\fZ}{\mathfrak{Z}}

\newcommand{\fa}{\mathfrak{a}}
\newcommand{\fb}{\mathfrak{b}}
\newcommand{\fc}{\mathfrak{c}}
\newcommand{\fd}{\mathfrak{d}}
\newcommand{\fe}{\mathfrak{e}}
\newcommand{\ff}{\mathfrak{f}}
\newcommand{\fg}{\mathfrak{g}}
\newcommand{\fh}{\mathfrak{h}}
%\newcommand{\fi}{\mathfrak{i}} % already defined!
\newcommand{\fj}{\mathfrak{j}}
\newcommand{\fk}{\mathfrak{k}}
\newcommand{\fl}{\mathfrak{l}}
\newcommand{\fm}{\mathfrak{m}}
\newcommand{\fn}{\mathfrak{n}}
\newcommand{\fo}{\mathfrak{o}}
\newcommand{\fp}{\mathfrak{p}}
\newcommand{\fq}{\mathfrak{q}}
\newcommand{\fr}{\mathfrak{r}}
\newcommand{\fs}{\mathfrak{s}}
\newcommand{\ft}{\mathfrak{t}}
\newcommand{\fu}{\mathfrak{u}}
\newcommand{\fv}{\mathfrak{v}}
\newcommand{\fw}{\mathfrak{w}}
\newcommand{\fx}{\mathfrak{x}}
\newcommand{\fy}{\mathfrak{y}}
\newcommand{\fz}{\mathfrak{z}}



% Sans Serif letters

\newcommand{\sA}{\mathsf{A}}
\newcommand{\sB}{\mathsf{B}}
\newcommand{\sC}{\mathsf{C}}
\newcommand{\sD}{\mathsf{D}}
\newcommand{\sE}{\mathsf{E}}
\newcommand{\sF}{\mathsf{F}}
\newcommand{\sG}{\mathsf{G}}
\newcommand{\sH}{\mathsf{H}}
\newcommand{\sI}{\mathsf{I}}
\newcommand{\sJ}{\mathsf{J}}
\newcommand{\sK}{\mathsf{K}}
\newcommand{\sL}{\mathsf{L}}
\newcommand{\sM}{\mathsf{M}}
\newcommand{\sN}{\mathsf{N}}
\newcommand{\sO}{\mathsf{O}}
\newcommand{\sP}{\mathsf{P}}
\newcommand{\sQ}{\mathsf{Q}}
\newcommand{\sR}{\mathsf{R}}
\newcommand{\sS}{\mathsf{S}}
\newcommand{\sT}{\mathsf{T}}
\newcommand{\sU}{\mathsf{U}}
\newcommand{\sV}{\mathsf{V}}
\newcommand{\sW}{\mathsf{W}}
\newcommand{\sX}{\mathsf{X}}
\newcommand{\sY}{\mathsf{Y}}
\newcommand{\sZ}{\mathsf{Z}}

\makeatother




%Tikz 
\usepackage{tikz}
\usetikzlibrary{decorations.markings,decorations.pathreplacing}%,external}
\tikzset{
->-/.style={decoration={markings, mark=at position .5 with {\arrow{>}}},postaction={decorate}},
-<-/.style={decoration={markings, mark=at position .5 with {\arrow{<}}},postaction={decorate}},
ARC/.style ={draw=black,line join=miter,line cap=butt,miter limit=4.00,line width=0.5 mm},
TEXTARC/.style ={draw=black,line join=miter,line cap=butt,miter limit=4.00,line width=0.3 mm},
REGION/.style={draw=none, fill=white!#1!black},
REGION/.default = 80,
}
%\tikzexternalize
%\tikzsetexternalprefix{figures/}

% The category of families of h-graphs with basepoints.
\newcommand{\calHbp}{\widetilde\calH}


% Environments for the axioms --- this fixes the vertical spacing.
\theoremstyle{definition}
\newtheorem*{BaseChange}{Base change}
\newtheorem*{Gluing}{Gluing}
\newtheorem*{Identity}{Identity}
\newtheorem*{Monoidality}{Monoidality}
\newtheorem*{Unit}{Unit}

% Command for FAMILIES.
\newcommand{\Fam}{\text{-}\mathrm{FAM}}

% External operations on families of cobordisms
\newcommand{\ucirc}{\mathbin{\underline{\circ}}}
\newcommand{\usqcup}{\mathbin{\underline{\sqcup}}}

% Ticks and crosses
\newcommand{\tickYes}{\checkmark}
\usepackage{pifont}
\newcommand{\tickNo}{\hspace{1pt}\ding{55}}

% Notation for the forgetful and inclusion functors
\newcommand{\forget}{\mathrm{forget}}
\newcommand{\inclusion}{\mathrm{incl}}
